Online Planning in POMDPs with Self-Improving Simulators

How can we plan efficiently in a large and complex environment when the time budget is limited? Given the original simulator of the environment, which may be computationally very demanding, we propose to learn online an approximate but much faster simulator that improves over time. To plan reliably and efficiently while the approximate simulator is learning, we develop a method that adaptively decides which simulator to use for every simulation, based on a statistic that measures the accuracy of the approximate simulator. This allows us to use the approximate simulator to replace the original simulator for faster simulations when it is accurate enough under the current context, thus trading off simulation speed and accuracy. Experimental results in two large domains show that when integrated with POMCP, our approach allows to plan with improving efficiency over time.

==> resubmission_cover_letter.tex <==
\onecolumn

\section*{Cover letter for resubmission}

\vspace{3pt}

\textbf{Title:} Online Planning in POMDPs with Self-Improving Simulators \vspace{5pt}

\noindent \textbf{Tracking number:} 7567 \vspace{5pt}

\noindent \textbf{Conference:} Thirty-Sixth AAAI Conference on Artificial Intelligence (AAAI-22) \vspace{5pt}

We received a very positive feedback from the meta reviewer: 
"We ultimately decided to recommend to reject the paper, but this
decision has been a very close one. Personally, I see more important
reasons to accept the paper (in particular the novelty and significance)
than to reject the paper, but our discussion showed that the paper fails
at delivering this impression properly."

The reviewers mainly had concerns on how far the proposed approach improves the existing two-phase approach, and found that the paper did not make sufficiently clear these benefits, both in writing, as well as in the experiments. In this version, we explicitly spell out the three drawbacks of the two-phase approach:
\begin{enumerate}
    \item the requirement of training an influence predictor to convergence prior to planning prevents the approach from being deployed directly. 
    \item there is a distribution shift issue when transferring the offline learned influence predictor to make online predictions during planning, which harms the planning performance.
    \item completely replacing with the global simulator with the approximate one after training implies a risk of very poor performance in certain situations.
\end{enumerate}

While point 1 is a qualitative feature that does not require demonstration, in this version, we also show experimentally how our approach mitigates 2 and 3. 


